Jet thermalization in QCD kinetic theory

We perform numerical studies in QCD kinetic theory to investigate the energy and angular profiles of a high energy parton - as a proxy for a jet produced heavy ion collisions - passing through a Quark-Gluon Plasma (QGP). We find that the fast parton loses energy to the plasma mainly via a radiative turbulent gluon cascade that transport energy locally from the jet down to the temperature scale where dissipation takes place. In this first stage, the angular structure of the turbulent cascade is found to be relatively collimated. However, when the lost energy reaches the plasma temperature is it rapidly transported to large angles w.r.t. the jet axis and thermalizes. We investigate the contribution of the soft jet constituents to the total jet energy. We show that for jet opening angles of about 0.3 rad or smaller the effect is negligible. Conversely, larger opening angles become more and more sensitive to the thermal component of the jet and thus to medium response. Our result showcase the importance of the jet cone size in mitigating or enhancing the details of dissipation in jet quenching observables.

==> HTL-Matrix.tex <==
In order to compute the QCD matrix element using HTL resummed propagators, 


\subsection{Gluon propagator}
The retarded gluon HTL propagator given by 
\begin{align}
    \label{eq:Retard}
    G^{00}_{R}(Q) &=& i G^{L}_R = \frac{i}{q^2 + m_D^2\left( 1- \frac{\omega}{2q} \left[ \log\left( \frac{q+\omega}{q-\omega} \right) - i\pi \right] \right)} \;,\\
    G^{ij}_{R}(Q) &=& i (\delta^{ij} - \hat{q}^i\hat{q}^j) G^{T}_R = \frac{i(\delta^{ij} - \hat{q}^i\hat{q}^j)}{\omega^2 - q^2 - m_D^2\left( \frac{\omega^2}{2q^2}- \frac{\omega}{4q} \left(\frac{\omega^2}{q^2}-1\right) \left[ \log\left( \frac{q+\omega}{q-\omega} \right) - i\pi \right]\right)} \;,
\end{align}
for $q>\omega$.

\subsection{Quark propagator}
The quark HTL self-energy is written 
\begin{eqnarray}
    \Sigma^0 (Q) &=& \frac{m_F^2}{2q} \left[ \ln\left( \frac{q+\omega}{q-\omega} \right) - i\pi \right]\;,\\
    \mathbf{\Sigma} (Q) &=& \hat{\q} \Sigma^T=- \hat{\q} \frac{m_F^2}{q} \left\{ 1-\frac{\omega}{2q}\left[\ln\left( \frac{q+\omega}{q-\omega} \right) - i\pi \right]\right\} \;,\\
\end{eqnarray}
with $m_F = gT\sqrt{C_F/8}$ and for $q>\omega$.
The propagator is then given by 
\begin{eqnarray}
    S_R(\mathcal{Q}) &=& \frac{\slashed{\mathcal{Q}}}{\mathcal{Q}\cdot\mathcal{Q}}\;,
\end{eqnarray}
where $\mathcal{Q} = Q^\mu - \Sigma^\mu(Q)$.

